Multigrid Methods using Block Floating Point Arithmetic

Block Floating Point (BFP) arithmetic is currently seeing a resurgence in interest because it requires less power, less chip area, and is less complicated to implement in hardware than standard floating point arithmetic. This paper explores the application of BFP to mixed- and progressive-precision multigrid methods, enabling the solution of linear elliptic partial differential equations (PDEs) in energy- and hardware-efficient integer arithmetic. While most existing applications of BFP arithmetic tend to use small block sizes, the block size here is chosen to be maximal such that matrices and vectors share a single exponent for all entries. This is sometimes also referred to as a scaled fixed-point format. We provide algorithms for BLAS-like routines for BFP arithmetic that ensure exact vector-vector and matrix-vector computations up to a specified precision. Using these algorithms, we study the asymptotic precision requirements to achieve discretization-error-accuracy. We demonstrate that some computations can be performed using as little as 4-bit integers, while the number of bits required to attain a certain target accuracy is similar to that of standard floating point arithmetic. Finally, we present a heuristic for full multigrid in BFP arithmetic based on saturation and truncation that still achieves discretization-error-accuracy without the need for expensive normalization steps of intermediate results.

==> setup.tex <==

\usepackage{color}
\usepackage[acronym,shortcuts]{glossaries}

%\usepackage{caption}
%\usepackage{subcaption}

\usepackage{pgf}
%\DeclareUnicodeCharacter{2212}{-}

% Packages and setup for pseudocode
\usepackage{algpseudocode} % for 'algorithmicx' which is an improved version of algorithmic
\usepackage{csquotes}

\usepackage{tikz}
\usetikzlibrary[arrows, decorations.pathmorphing, backgrounds, patterns, positioning, fit, petri]

\usepackage{siunitx}
\sisetup{output-exponent-marker=\ensuremath{\mathrm{e}}}

\usepackage[symbol]{footmisc}

\usepackage{booktabs}

\usepackage{makecell}
\renewcommand{\cellalign}{tl}

%%%%%%%%%%%%%%%%%%%
%% Theorem setup %%
%%%%%%%%%%%%%%%%%%%

\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

%%%%%%%%%%%%%%%%%%%%%
%% Algorithm setup %%
%%%%%%%%%%%%%%%%%%%%%

% Used for all algorithms
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Precondition:}}
% \Comment[<len>]{<stuff>} is reformatted to put the comment <stuff> in a box of width <len> (default is .5\linewidth) flush right.
\algrenewcommand{\algorithmiccomment}[2][.6\linewidth]{\leavevmode\hfill\makebox[#1][l]{\textcolor{darkgray}{$\triangleright$ #2}}}
\algnewcommand{\algorithmicgoto}{\textbf{goto}}%!TEX encoding = UTF-8 Unicode
\algnewcommand{\Goto}[1]{\algorithmicgoto~\ref{#1}}%
\algnewcommand\algorithmicvariables{\textbf{Local variables:}}%
\algnewcommand\Variables{\item[\algorithmicvariables]}%

% Declaration of the new block
\algblock{ParFor}{EndParFor}
% Customising the new block
\algnewcommand\algorithmicparfor{\textbf{parallel for}}
\algnewcommand\algorithmicpardo{\textbf{do}}
\algnewcommand\algorithmicendparfor{\textbf{end\ parallel for}}
\algrenewtext{ParFor}[1]{\algorithmicparfor\ #1\ \algorithmicpardo}
\algrenewtext{EndParFor}{\algorithmicendparfor}

\algnewcommand{\LineComment}[1]{\vspace{3pt}\Statex \(\triangleright\)\(\triangleright\) \textcolor{blue}{#1} \vspace{3pt}}
\newcommand{\COMMENT}[2][.47\linewidth]{%
    \leavevmode\hfill\makebox[#1][l]{$\triangleright$~#2}}

%%%%%%%%%%%
%% TODOs %%
%%%%%%%%%%%

\newcommand{\nk}[1]{\textcolor{red}{\textbf{Nils}:~#1}}
\newcommand{\rt}[1]{\textcolor{red}{\textbf{Rasmus}:~#1}}
\newcommand{\sm}[1]{\textcolor{red}{\textbf{Steve}:~#1}}


%%%%%%%%%%%%
%% Macros %%
%%%%%%%%%%%%

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\ir}{$\mathcal{IR}$}
\newcommand{\V}{$\mathcal{V}$}
\newcommand{\fmg}{$\mathcal{FMG}$}
\newcommand{\s}{$\mathcal{S}$}

\newcommand{\exact}[1]{{#1}^\ast}
\newcommand{\bfptfont}[1]{\mathsf{#1}}

\newcommand{\Q}[2]{Q_{#1.#2}} % Q format
\newcommand{\powersoftwo}{\mathfrak{P}_2}
\newcommand{\rep}{\mathtt{rep}}

\newcommand{\bfp}{\mathbb{B}}
\newcommand{\bfpm}[1]{#1_m} % block-float "mantissa vector"
\newcommand{\bfpe}[1]{#1_e} % block-float exponent
\newcommand{\bfpq}[1]{#1_w} % block-float mantissa length
\newcommand{\bfpd}[1]{#1_d} % block-float dimension(s)
\newcommand{\bfpt}[1]{(\bfpe{#1}, \bfpm{#1}, \bfpq{#1}, \bfpd{#1})} % block-float tuple
\newcommand{\bfpequal}{\sim}

\newcommand{\LeftShift}{\ll}
\newcommand{\RightShift}{\gg}
\newcommand{\trunc}[2]{\text{trunc}\left(#1, #2 \right)}

\newcommand{\bfpn}[1]{\text{bfpnorm}\left(#1\right)} % BFP normalization
\newcommand{\bfpset}[2]{\signed \times \left[\Q{1}{#1}\right]^{#2}}
\newcommand{\bfpsetnopow}[2]{\left[\Q{1}{#1}\right]^{#2}} % BFP normalization

\newcommand{\real}{\mathbb{R}}
\newcommand{\unsigned}{\mathbb{Z}_{\geq 0}}
\newcommand{\unsignedpositive}{\mathbb{Z}_{> 0}}
\newcommand{\signed}{\mathbb{Z}}
\newcommand{\rational}{\mathbb{Q}}
\newcommand{\twoscomp}[1]{\mathbb{X}_{#1}}     % integer range for bit-width w (twos complement)
\newcommand{\fixed}[2]{\mathbb{F}_{(#1, #2)}} % fixed-point numbers with bit-width w and scaling factor f

\newcommand{\round}{\bigcirc}                 % rounding
\newcommand{\roundzero}{\bigcirc}                 % rounding towards zero

\newcommand{\quant}[1]{\text{quant}_{#1}}        % quantization

\newcommand{\tmp}[1]{{#1}_\textrm{tmp}}                 % temporary variable
\newcommand{\out}[1]{{#1}_\textrm{out}}                 % output variable

\newcommand{\dinva}{\tilde{A}}
\newcommand{\dinvb}{\tilde{b}}

\newcommand{\ewe}{\boldsymbol{\varepsilon}}
\newcommand{\ewed}{\boldsymbol{\dot{\varepsilon}}}
\newcommand{\eweb}{\boldsymbol{\bar{\varepsilon}}}
\newcommand{\eweq}{\boldsymbol{\check{\varepsilon}}}

\newcommand{\wewe}{w}
\newcommand{\wewed}{\dot{w}}
\newcommand{\weweb}{\bar{w}}
\newcommand{\weweq}{\check{w}}

%%%%%%%%%%%%
%% Colors %%
%%%%%%%%%%%%

\definecolor{ColorNeutralBits}{RGB}{35, 87, 137}
\definecolor{ColorEnoughBits}{RGB}{59, 178, 115}
\definecolor{ColorOverflow}{RGB}{239, 48, 84}
\definecolor{ColorUnderflow}{RGB}{255, 111, 89}

\definecolor{lo}{HTML}{33A02C}
\definecolor{med}{HTML}{1F78B4}
\definecolor{hi}{HTML}{E31A1C}

\definecolor{lo_light}{HTML}{B2DF8A}
\definecolor{med_light}{HTML}{A6CEE3}
\definecolor{hi_light}{HTML}{FB9A99}
\definecolor{quant}{HTML}{FF7F00}

%%%%%%%%%%%%%%
%% Acronyms %%
%%%%%%%%%%%%%%

\newacronym{bfp}{BFP}{block floating point}
\newacronym{blas}{BLAS}{Basic Linear Algebra Subprograms}
\newacronym{fmg}{FMG}{full multigrid}
% \newacronym{ir}{\ir}{iterative refinement}
\newacronym{msb}{MSB}{most significant bit}
\newacronym{lsb}{LSB}{least significant bit}
\newacronym{pde}{PDE}{partial differential equation}
\newacronym{spd}{SPD}{symmetric positive definite}

